Automated Remote Sensing Forest Inventory Using Satellite Imagery

For many countries like Russia, Canada, or the USA, a robust and detailed tree species inventory is essential to manage their forests sustainably. Since one can not apply unmanned aerial vehicle (UAV) imagery-based approaches to large-scale forest inventory applications, the utilization of machine learning algorithms on satellite imagery is a rising topic of research. Although satellite imagery quality is relatively low, additional spectral channels provide a sufficient amount of information for tree crown classification tasks. Assuming that tree crowns are detected already, we use embeddings of tree crowns generated by Autoencoders as a data set to train classical Machine Learning algorithms. We compare our Autoencoder (AE) based approach to traditional convolutional neural networks (CNN) end-to-end classifiers.

==> tables/2DCNNtable1.tex <==
\begin{table}[!htbp]
\centering\caption{Accuracy for every label, overall accuracy, and overall F1 score for all considered image sizes on the train/test set. Results in bold indicates the highest achieved value.\label{table2}}
\begin{tabular}{|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|}
\hline
 & \tiny $\boldsymbol{10\times 10}$ & \tiny $\boldsymbol{14\times 14}$ & \tiny $\boldsymbol{18\times 18}$ & \tiny $\boldsymbol{22\times 22}$ & \tiny $\boldsymbol{26\times 26}$ & \tiny $\boldsymbol{30\times 30}$  	 \\ 
 \hline 
\tiny \textbf{Acc. Label 0} & \tiny 37.42  & \tiny 47.1 & \tiny 45.8 & \tiny 47.7 & \tiny \textbf{52.3} & \tiny 49	 \\ 
\hline
\tiny \textbf{Acc. Label 1}  & \tiny \textbf{69.47} & \tiny 64.21 & \tiny 60 & \tiny 60.11 & \tiny 61.1 & \tiny 51.6 	 \\
\hline
\tiny \textbf{Acc. Label 2}  & \tiny 69.23 & \tiny 61.54 & \tiny \textbf{76.9} & \tiny 46.2 & \tiny 53.8 & \tiny 46.42  	 \\
\hline
\tiny \textbf{Acc. Label 3}  & \tiny 92.68 & \tiny 92.68 & \tiny \textbf{92.7} & \tiny 95.1 & \tiny 95.16 &\tiny  95.12 	 \\
\hline
\tiny \textbf{Overall Acc.} & \tiny 56.25 & \tiny 60.3 & \tiny \tiny 57.89 & \tiny 58.55 & \tiny \textbf{60.7} & \tiny 55.90 	 \\
\hline
\tiny \textbf{Overall F1} & \tiny 0.55 & \tiny \textbf{0.576} & \tiny 0.563 & \tiny 0.548 & \tiny 0.56 & \tiny 0.53 	 \\
\hline 
\end{tabular}
\end{table}


==> tables/SAtable1.tex <==

\begin{table}[!htbp]
\centering
\caption{Highest achieved accuracy for combinations of bottleneck and image sizes using coordinates as additional features on the train/test set.
}
\begin{tabular}{|@{ }c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|}
\hline
& \tiny\textbf{40} & \tiny\textbf{60} & \tiny\textbf{80} & \tiny\textbf{100}& \tiny\textbf{120} \\ 
\hline
\tiny $\boldsymbol{10\times 10}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny CatB.:\\ \tiny 0.99/0.719\end{tabular}\endgroup & 
\textbf{\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny CatB.: \\ \tiny 0.99/0.739 \end{tabular}\endgroup} & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.719\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.734\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.714\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{14\times 14}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.93/0.734\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.685\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.714\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.729\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.714\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{18\times 18}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.95/0.685\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny 0.99/0.675\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.99/0.7\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.99/0.685 \end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.69\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{22\times 22}$    & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.96/0.69\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.685\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.655\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.65\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.67\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{26\times 26}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.67\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.65\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.616\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.66\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.99/0.67\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{30\times 30}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny 0.99/0.631\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.635\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.67\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.635\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.99/0.635\end{tabular}\endgroup \\ 
\hline
\end{tabular}
\end{table}

==> tables/SAtable2.tex <==
\begin{table}[!htbp]
\centering
\caption{Highest achieved accuracy for combinations of bottleneck and image sizes without using coordinates as additional features on the train/test set.}
\begin{tabular}{|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|}
\hline
& \tiny \textbf{40} & \tiny \textbf{60} & \tiny \textbf{80} & \tiny \textbf{100}& \tiny \textbf{120} \\ 
\hline

\tiny $\boldsymbol{10\times 10}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.739\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.724\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.724\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.714\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.719\end{tabular}\endgroup \\ 
\hline

\tiny $\boldsymbol{14\times 14}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.704\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.719\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.734\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.719\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.68\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{18\times 18}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\\tiny 0.99/0.695\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\\tiny 0.99/0.665\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\\tiny 0.99/0.7\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\\tiny 0.99/0.709 \end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\\tiny 0.99/0.709\end{tabular}\endgroup \\ \hline
\tiny $\boldsymbol{22\times 22}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.64\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.655\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.68\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.675\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.695\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{26\times 26}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC:\\ \tiny  0.99/0.616\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.66\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\ \tiny 0.99/0.66\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.665\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.66\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{30\times 30}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny 0.99/0.596\end{tabular}\endgroup &
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny 0.99/0.645\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.665\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.645\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\ \tiny 0.99/0.616\end{tabular}\endgroup \\ 
\hline
\end{tabular}
\end{table}

==> tables/SAtable3.tex <==
\begin{table}[!htbp]
\centering
\caption{Highest achieved F1-score for combinations of bottleneck and image sizes using coordinates as additional features on the train/test set. \label{F8table}
}
\begin{tabular}{|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|}
\hline
& \tiny \textbf{40} & \tiny \textbf{60} & \tiny \textbf{80} & \tiny \textbf{100} & \tiny \textbf{120} \\ 
\hline
\tiny $\boldsymbol{10\times 10}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny 0.99/0.57\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.565\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.558\end{tabular}\endgroup  & 
\textbf{\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.62\end{tabular}\endgroup } & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny \tiny CatB.: \\ \tiny 0.99/0.548\end{tabular}\endgroup  \\ 
\hline
\tiny $\boldsymbol{14\times 14}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.93/0.609\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.529\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.546\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.61\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.594\end{tabular}\endgroup  \\ 
\hline
\tiny $\boldsymbol{18\times 18}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.95/0.536\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny 0.99/0.507\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.99/0.538\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.99/0.523\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.509\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{22\times 22}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.96/0.532\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.555\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.486\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.486\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.508\end{tabular}\endgroup  \\ 
\hline
\tiny $\boldsymbol{26\times 26}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.501\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.489\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.473\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.492\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.99/0.564\end{tabular}\endgroup  \\ 
\hline
\tiny $\boldsymbol{30\times 30}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny 0.99/0.463\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.491\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.513\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.493\end{tabular}\endgroup  & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.99/0.498\end{tabular}\endgroup  \\
\hline
\end{tabular}
\end{table}


==> tables/SAtable4.tex <==
\begin{table}[!htbp]
\centering
\caption{Highest achieved F1-score for combinations of bottleneck and image sizes without using coordinates as additional features on the train/test set.\label{F9table}
}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|}
\hline
& \tiny \textbf{40} & \tiny \textbf{60} & \tiny \textbf{80} & \tiny \textbf{100} & \tiny \textbf{120} \\ \hline
\tiny $\boldsymbol{10\times 10}$ & 
\textbf{\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.62\end{tabular}\endgroup} & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.606\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.551\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.554\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny 0.99/0.562\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{14\times 14}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.539\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.541\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.608\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.551\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny  0.97/0.571\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{18\times 18}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.523\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.504\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny  0.99/0.532\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\ \tiny  0.99/0.537\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\ \tiny  0.99/0.543\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{22\times 22}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.484\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.505\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.513\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.518\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.528\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{26\times 26}$ & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny  0.99/0.447\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.502\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\ \tiny  0.99/0.498\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.552\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.49\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{30\times 30}$ & \begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny  0.999/0.43\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny RFC: \\ \tiny  0.99/0.468\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.506\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny CatB.: \\ \tiny  0.99/0.489\end{tabular}\endgroup & 
\begingroup\renewcommand{\arraystretch}{0.7}\begin{tabular}{@{}c@{}}\tiny XGB: \\ \tiny  0.99/0.513\end{tabular}\endgroup \\ 
\hline
\end{tabular}
\end{table}

==> tables/appendAtable1.tex <==

\begin{table}[!htb]

\centering
\caption{Accuracy scores of the best classifiers for give bottleneck values and image size on the train/test set. Vertical columns stands for image size and horizontal one for bottleneck size.  \label{Accuracytable}
}

\begin{tabular}{|@{ }c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|}
\hline
& \tiny\textbf{40} & \tiny \textbf{60} & \tiny \textbf{80} & \tiny \textbf{100} & \tiny \textbf{120} \\ \hline
\tiny $\boldsymbol{10\times 10}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny SVC:\\ \tiny 0.96/0.753\end{tabular}\endgroup & \textbf{\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.768\end{tabular}\endgroup} & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.97/0.743\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny CatB.:\\ \tiny  0.99/0.763\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.768\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{14\times 14}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny SVC:\\ \tiny 0.97/0.738\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny SVC:\\ \tiny 0.98/0.768\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.758\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.97/0.748\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.98/0.733\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{18\times 18}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.699\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.98/0.753\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.748\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.714\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.733\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{22\times 22}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny  SVC: \\ \tiny  0.97/0.719\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.729\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\\tiny  0.98/0.729\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.743\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.99/0.748\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{26\times 26}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.97/0.650\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.689\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.719\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.99/0.743\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.99/0.709\end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{30\times 30}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.97/0.674\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.669\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.714\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.99/0.724\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.99/0.733\end{tabular}\endgroup \\ \hline


\end{tabular}
\end{table}




==> tables/appendxAtable2.tex <==
\begin{table}[!htb]
\centering
\caption{F1 scores of the best classifiers for give bottleneck values and image size on the train/test set. Vertical columns stands for image size and horizontal one for bottleneck size. \label{F7table}
}

\begin{tabular}{|@{ }c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|@{}c@{ }|}
\hline
& \tiny\textbf{40} & \tiny \textbf{60} & \tiny \textbf{80}& \tiny \textbf{100}& \tiny \textbf{120} 
\\ \hline
\tiny $\boldsymbol{10\times 10}$ &
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny SVC:\\ \tiny 0.96/0.636 \tiny \end{tabular}\endgroup &
\textbf{\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.645   \tiny \end{tabular}\endgroup} &
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.97/0.631 \tiny \end{tabular}\endgroup &
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.639 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.645 \end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{14\times 14}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny SVC:\\ \tiny 0.97/0.571 \tiny \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}} \tiny SVC:\\ \tiny 0.98/0.6 \tiny \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.59 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.588 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.91/0.581 \end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{18\times 18}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.54 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC: \\ \tiny 0.98/0.586\end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.575 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.556 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.99/0.574 \end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{22\times 22}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny  SVC: \\ \tiny 0.97/0.551 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.55 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.566 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.574 \end{tabular} \endgroup& \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.99/0.576 \end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{26\times 26}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.509  \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.536 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.555  \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.99/0.577 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.99/0.551 \end{tabular}\endgroup \\ 
\hline
\tiny $\boldsymbol{30\times 30}$ & 
\begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.97/0.529 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.98/0.516 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny  0.98/0.552  \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny0.99/0.551 \end{tabular}\endgroup & \begingroup\renewcommand{\arraystretch}{0.7} \begin{tabular}{@{}c@{}}\tiny SVC:\\ \tiny 0.99/0.561  \end{tabular}\endgroup\\ 
\hline
\end{tabular}
\end{table}

